Strategic Negotiations in Endogenous Network Formation

In network formation games, agents form edges with each other to maximize their utility. Each agent's utility depends on its private beliefs and its edges in the network. Strategic agents can misrepresent their beliefs to get a better resulting network. Most prior works in this area consider honest agents or a single strategic agent. Instead, we propose a model where any subset of agents can be strategic. We provide an efficient algorithm for finding the set of Nash equilibria, if any exist, and certify their nonexistence otherwise. We also show that when several strategic agents are present, their utilities can increase or decrease compared to when they are all honest. Small changes in the inter-agent correlations can cause such shifts. In contrast, the simpler one-strategic-agent setting explored in the literature lacks such complex patterns. Finally, we develop an algorithm by which new agents can learn the information needed for strategic behavior. Our algorithm works even when the (unknown) strategic agents deviate from the Nash-optimal strategies. We verify these results on both simulated networks and a real-world dataset on international trade.

==> checklist.tex <==
\section{Reproducibility Checklist}

Unless specified otherwise, please answer “yes” to each question if the relevant information is described either in the paper itself or in a technical appendix with an explicit reference from the main paper. If you wish to explain an answer further, please do so in a section titled “Reproducibility Checklist” at the end of the technical appendix.

This paper:

Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes/partial/no/NA)

{\bf Yes.}

Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes/no)

{\bf Yes.}

Provides well marked pedagogical references for less-familiar readers to gain background necessary to replicate the paper (yes/no)

{\bf Yes.}

Does this paper make theoretical contributions? (yes/no)

{\bf Yes.}

If yes, please complete the list below.

All assumptions and restrictions are stated clearly and formally. (yes/partial/no)

{\bf Yes.}

All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)

{\bf Yes.}

Proofs of all novel claims are included. (yes/partial/no)

{\bf Yes.}

Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)

{\bf Yes.}

Appropriate citations to theoretical tools used are given. (yes/partial/no)

{\bf Yes.}

All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)

{\bf Yes.}


All experimental code used to eliminate or disprove claims is included. (yes/no/NA)

{\bf Yes.}

Does this paper rely on one or more datasets? (yes/no)

{\bf Yes.}

If yes, please complete the list below.

A motivation is given for why the experiments are conducted on the selected datasets (yes/partial/no/NA)

{\bf Yes.}

All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/NA)

{\bf NA (No new datasets).}

All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/NA)

{\bf NA (No new datasets).}

All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes/no/NA)

{\bf Yes.}

All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes/partial/no/NA)

{\bf Yes.}

All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/NA)

{\bf NA (Data are publicly available).}

Does this paper include computational experiments? (yes/no)

{\bf Yes.}

If yes, please complete the list below.

Any code required for pre-processing data is included in the appendix. (yes/partial/no).

{\bf Yes.}

All source code required for conducting and analyzing the experiments is included in a code appendix. (yes/partial/no)

{\bf Yes.}

All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no)

{\bf Yes.}

All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes/partial/no)

{\bf Yes.}

If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/NA)

{\bf Yes.}

This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes/partial/no)

{\bf Yes.}

This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes/partial/no)

{\bf Yes.}

This paper states the number of algorithm runs used to compute each reported result. (yes/no)

{\bf Yes.}

Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/no)

{\bf Yes.}

The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/no)

{\bf Yes.}

This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes/partial/no/NA)

{\bf Yes.}


This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes/partial/no/NA)

{\bf Yes.}

